VERDICT: Verifiable Evolving Reasoning with Directive-Informed Collegial Teams for Legal Judgment Prediction

Legal Judgment Prediction (LJP) predicts applicable law articles, charges, and penalty terms from case facts. Beyond accuracy, LJP calls for intrinsically interpretable and legally grounded reasoning that can reconcile statutory rules with precedent-informed standards. However, existing methods often behave as static, one-shot predictors, providing limited procedural support for verifiable reasoning and little capability to adapt as jurisprudential practice evolves. We propose VERDICT, a self-refining collaborative multi-agent framework that simulates a virtual collegial panel. VERDICT assigns specialized agents to complementary roles (e.g., fact structuring, legal retrieval, opinion drafting, and supervisory verification) and coordinates them in a traceable draft--verify--revise workflow with explicit Pass/Reject feedback, producing verifiable reasoning traces and revision rationales. To capture evolving case experience, we further introduce a Hybrid Jurisprudential Memory (HJM) grounded in the Micro-Directive Paradigm, which stores precedent standards and continually distills validated multi-agent verification trajectories into updated Micro-Directives for continual learning across cases. We evaluate VERDICT on CAIL2018 and a newly constructed CJO2025 dataset with a strict future time-split for temporal generalization. VERDICT achieves state-of-the-art performance on CAIL2018 and demonstrates strong generalization on CJO2025. To facilitate reproducibility and further research, we release our code and the dataset at https://anonymous.4open.science/r/ARR-4437.

==> sections/1.introduction_old.tex <==
\section{Introduction}
% 先  需要提出重要性 困难 数字  全世界多少案件需要审理  现有人工体系不堪重负
% 再 LJP旨在使用人工智能方法帮助..然而 法律案件存在..问题 所以 .. 是困难的  
% 法律判决预测（LJP）是智能司法系统的核心应用，旨在根据案件事实预测法条、罪名及刑期，以提升司法效率与一致性 \citep{zhong2018topjudge}。然而，由于法律逻辑的复杂性与司法标准的（） ，实现严谨且可解释的裁决极具挑战。

%  现有方法 表层特征 deep 不能说OOD 说缺乏深层法理思考 和 普遍案件的泛化  解释标准 规则 各个国家实际..
% 现有方法主要面临两大瓶颈。判别式模型（从 CNN 到图网络）虽然在静态基准上表现尚可，但往往退化为依赖高频文本模式的“捷径学习”，导致在分布外（OOD）场景下泛化能力骤降。另一方面，生成式大语言模型（LLM）虽然语义理解力强，但存在幻觉与逻辑松散问题。简单的检索增强（RAG）仅能提供法条依据，却无法像人类法官那样，弥合“刚性规则（Rules）”与“模糊标准（Standards）”之间的鸿沟。目前的系统缺乏在实践中持续积累经验的“认知成长”机制，训练完成后便陷入静态，无法适应复杂的法理演变。
% 为了突破上述局限，我们提出了 SRM-LJP（自修正多智能体框架）。这是一个模拟中国刑事案件庭审“合议庭”的协作系统，其设计核心在于将计算法学中的“微观指令范式”实体化。面对“规则”与“标准”的权衡，我们认为理想的 AI 应具备从海量先例中提炼“中间层智慧”的能力。为此，我们构建了混合法理记忆（HJM），模拟人类法官的认知成长过程。该系统通过“归纳生成”与“对比细化”的持续循环，从原始先例中动态蒸馏出“微观指令（Micro-Directives）”。这些指令构成了介于抽象法条与具体个案之间、具有实操指导意义的裁判经验，从而赋予了模型持续学习与精准推理的能力。
Legal Judgment Prediction (LJP), which aims to automatically predict law articles, charges, and penalty terms based on case facts, serves as a pivotal application in intelligent judicial systems. It promises to assist legal practitioners by enhancing efficiency and ensuring consistency across rulings \citep{zhong2018topjudge}. However, achieving rigorous and explainable adjudication remains a formidable challenge due to the complexity of legal logic and the dynamic evolution of judicial standards.

Existing approaches face two primary bottlenecks. \textbf{Discriminative models}, ranging from early text classifiers \citep{kim2014convolutional} to recent graph networks \citep{yue2021neurjudge}, often degenerate into shortcut learning—relying on high-frequency textual patterns rather than legal reasoning. Consequently, they suffer from poor generalization in \textit{Out-of-Distribution (OOD)} scenarios. On the other hand, \textbf{Generative Large Language Models (LLMs)}, while possessing strong semantic understanding, are plagued by \textit{hallucination} and \textit{logical looseness}. Simple Retrieval-Augmented Generation (RAG) can provide statutory grounds but fails to bridge the jurisprudential gap between rigid \textbf{Rules} (statutes) and flexible \textbf{Standards} (precedents) \citep{kaplow2013rules} akin to human judges.\\

%这之后说 尽管已经有些探索 但是依然存在三个问题  
% 1.现有方法可解释性不强，分类模型直接预测结果，pljp用llm，但只用来生成答案 缺推理过程法理分析 法律领域 可解释性 非常重要（引一个法律文章）
% 2.存在非常多语义相似但法理不同的易混淆，如何精准识别案件和法条之间的关联性
% 3.法律领域 经验 先例 重要 过去方法缺乏经验利用  简单RAG不足  如何存储经验  以及后续调用 

Current systems lack the \textbf{cognitive growth} mechanism for accumulating experience in practice, remaining static after training and unable to adapt to complex legal evolution.
\begin{figure*}[t] 
    \centering
    \includegraphics[width=1.0\textwidth]{figs/framework.pdf} 
    \caption{\textbf{The overall architecture of SRM-LJP.} The system simulates a ``Virtual Collegial Panel'' workflow. (Left) The Clerk and Assistant retrieve facts and statutes. (Middle) The Case Judge drafts an initial judgment based on statutes, which is then scrutinized by the Supervisor using the Hybrid Jurisprudential Memory (HJM). (Right) The Presiding Judge issues the final verdict. The example shows how the system corrects a charge from ``Intentional Injury'' to ``Picking Quarrels'' based on micro-directives.}
    \label{fig:framework} 
\end{figure*}
\\
% 一段说自己的方法 
To address these limitations, we present \textbf{SRM-LJP} (Self-Refining Multi-Agent Framework,Figure \ref{fig:framework}) , a collaborative system simulating the "Collegial Panel" in Chinese criminal trials. Our design core lies in \textbf{operationalizing the "Micro-Directive Paradigm"} from computational law \citep{casey2016death}. Facing the trade-off between Rules and Standards, we posit that an ideal AI should possess the capability to distill \textbf{intermediate wisdom} from massive precedents. To this end, we construct a \textbf{Hybrid Jurisprudential Memory (HJM)} that mimics the cognitive growth process of human judges. Through continuous cycles of Inductive Generation and Contrastive Refinement, the system dynamically distills \textbf{Micro-Directives} from raw precedents. These directives constitute practical adjudication norms bridging abstract statutes and specific cases, thereby endowing the model with capabilities for continuous learning and precise reasoning.

% 为了严谨评估模型的时间鲁棒性，我们构建了一个纯净的分布外（OOD）数据集 CJO2025，其中包含 2025 年 1 月 1 日之后判决的案件。这确保了相对于大语言模型的预训练语料库，该数据实现了“零污染”。
% 本文的主要贡献总结如下：
% 我们提出了 SRM-LJP，这是一个拓扑多智能体框架。它通过程序感知指令微调和基于 DPO（直接偏好优化）的自修正机制，将通用大语言模型与严谨的司法逻辑对齐。
% 我们设计了一种混合法理记忆（HJM）来模拟法官的认知成长。通过从案件轨迹中提炼“微指令（Micro-Directives）”，该机制赋予了系统持续学习的能力。
% 我们发布了 CJO2025，这是一个用于测试时间泛化能力的新型未来切分（future-split）数据集。大量实验表明，SRM-LJP 在标准设置和 OOD 设置下均显著优于现有的 SOTA 基线模型。

To rigorously evaluate our model's temporal robustness, we construct a pristine OOD dataset, \textbf{CJO2025}, comprising cases adjudicated after January 1, 2025. This ensures zero data contamination relative to the LLM's pre-training corpus.
The main contributions of this work are summarized as follows:
\begin{itemize}
    \item We propose SRM-LJP, a topological multi-agent framework that aligns general LLMs with rigorous judicial logic through protocol-aware instruction tuning and DPO-based self-refining.
    \item We design a Hybrid Jurisprudential Memory (HJM) that simulates cognitive growth. By distilling "Micro-Directives" from case trajectories, it endows the system with continuous learning capabilities.
    \item We release CJO2025, a novel future-split dataset for testing temporal generalization. Extensive experiments show that SRM-LJP significantly outperforms SOTA baselines in both standard and OOD settings.
\end{itemize}

==> sections/3.problem_formulation.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
    \begin{tabular}{rl|ccccc|ccccc|cccc}
    \hline
    \multicolumn{2}{c|}{\multirow{2}{*}{}} & \multicolumn{5}{c|}{\textbf{Law Article}} & \multicolumn{5}{c|}{\textbf{Charge}} & \multicolumn{4}{c}{\textbf{Term of Penalty}} \\
    \multicolumn{2}{c|}{} & \textbf{Acc\%} & \textbf{MP\%} & \textbf{MR\%} & \textbf{F1\%} & \textbf{Hit@2} & \textbf{Acc\%} & \textbf{MP\%} & \textbf{MR\%} & \textbf{F1\%} & \textbf{Hit@2} & \textbf{Acc\%} & \textbf{MP\%} & \textbf{MR\%} & \textbf{F1\%} \\
    \hline
    1 & CNN & 69.52 & 62.14 & 58.35 & 60.18 & 74.15 & 73.56 & 70.45 & 65.23 & 67.74 & 79.66 & 33.24 & 28.56 & 25.14 & 26.74 \\
    2 & BERT & 76.54 & 73.21 & 70.45 & 71.80 & 81.87 & 75.85 & 78.45 & 76.12 & 77.26 & 82.25 & 29.80 & 32.14 & 29.56 & 30.79 \\
    \hline
    3 & MLAC & 73.02 & 69.27 & 66.14 & 64.23 & 79.54 & 74.73 & 72.65 & 69.56 & 68.36 & 81.27 & 36.45 & 34.50 & 29.95 & 29.64 \\
    4 & TOPJUDGE & 78.60 & 76.59 & 74.84 & 73.72 & 84.31 & 81.17 & 81.87 & 80.57 & 79.96 & 86.13 & 35.70 & 32.81 & 31.03 & 31.49 \\
    5 & MPBFN & 76.83 & 74.57 & 71.45 & 70.57 & 82.29 & 76.17 & 78.88 & 75.65 & 75.68 & 84.33 & 36.18 & 33.67 & 30.08 & 29.43 \\
    6 & EPM & \underline{83.98} & 80.82 & 77.55 & 78.10 & 88.17 & 79.10 & \underline{84.55} & 80.22 & \underline{81.43} & 86.52 & 36.69 & \underline{35.60} & 32.70 & 32.99 \\
    \hline
    7 & LADAN & 78.70 & 74.95 & 75.61 & 73.83 & 85.30 & 80.86 & 81.69 & 80.40 & 80.05 & 86.92 & 36.14 & 31.85 & 29.67 & 29.28 \\
    8 & NeurJudge & 78.74 & 80.34 & \underline{81.92} & \underline{79.66} & 86.06 & 79.04 & 82.60 & \textbf{80.92} & 80.70 & \underline{87.40} & 37.44 & 34.07 & 32.77 & 31.94 \\
    9 & R-former & 79.75 & 70.69 & 72.91 & 70.73 & 87.79 & 69.89 & 59.91 & 68.46 & 62.79 & 84.20 & \textbf{40.08} & 32.31 & \textbf{36.00} & \underline{33.39} \\
    10 & CTM & 81.72 & 79.67 & 77.67 & 76.82 & 85.79 & \underline{81.22} & 77.51 & 78.17 & 77.99 & 87.13 & 37.35 & 32.17 & 29.15 & 30.57 \\
    11 & PLJP & 83.21 & \underline{84.62} & 79.47 & 74.87 & \underline{89.21} & 79.32 & 76.84 & 74.32 & 76.32 & 86.20 & 36.84 & 34.80 & 32.22 & 32.48 \\
    \hline
    12 & OURS & \textbf{85.35} & \textbf{88.82} & \textbf{82.07} & \textbf{83.29} & \textbf{93.49} & \textbf{82.40} & \textbf{89.33} & \underline{80.89} & \textbf{82.36} & \textbf{90.64} & \underline{39.76} & \textbf{35.77} & \underline{33.98} & \textbf{34.08} \\
    \hline
    \end{tabular}%
}
\caption{Comparisons with the SOTA models on CAIL2018.}
\label{tab:sota-comparison-cail2018}
\end{table*}

\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
    \begin{tabular}{rl|ccccc|ccccc|cccc}
    \hline
    \multicolumn{2}{c|}{\multirow{2}{*}{}} & \multicolumn{5}{c|}{\textbf{Law Article}} & \multicolumn{5}{c|}{\textbf{Charge}} & \multicolumn{4}{c}{\textbf{Term of Penalty}} \\
    \multicolumn{2}{c|}{} & \textbf{Acc\%} & \textbf{MP\%} & \textbf{MR\%} & \textbf{F1\%} & \textbf{Hit@2} & \textbf{Acc\%} & \textbf{MP\%} & \textbf{MR\%} & \textbf{F1\%} & \textbf{Hit@2} & \textbf{Acc\%} & \textbf{MP\%} & \textbf{MR\%} & \textbf{F1\%} \\
    \hline
    1 & TOPJUDGE & 71.30 & 68.89 & 74.2 & 71.28 & 80.35 & 72.19 & 71.82 & 69.45 & 70.53 & 83.26 & 36.83 & 27.45 & 24.96 & 26.10 \\
    2 & EPM & 75.23 & 76.45 & 74.89 & 76.10 & 87.77 & 73.42 & 74.15 & 69.88 & 72.20 & 85.72 & 43.44 & 25.10 & 28.77 & 26.65 \\
    \hline
    3 & LADAN & 71.23 & 72.45 & 70.98 & 71.12 & 85.70 & 70.23 & 71.45 & 69.89 & 70.67 & 84.10 & 37.92 & 28.32 & 27.70 & 27.14 \\
    4 & NeurJudge & 73.69 & 74.4 & 80.14 & 72.44 & 84.20 & 74.30 & 71.59 & 77.5 & 70.56 & 86.17 & 42.87 & 25.40 & 26.37 & 25.14 \\
    5 & R-former & 75.00 & 62.04 & 69.70 & 62.90 & 86.56 & 68.07 & 48.93 & 59.19 & 50.76 & 79.80 & \underline{45.48} & 24.27 & \textbf{30.97} & 26.29 \\
    6 & CTM & 76.71 & 68.30 & 71.07 & 69.57 & 83.18 & 73.17 & 72.25 & 71.40 & 70.31 & 85.18 & 41.17 & 24.50 & 26.67 & 25.33 \\
    7 & PLJP & 86.30 & \underline{87.23} & \underline{83.25} & \underline{85.50} & \underline{90.33} & \underline{83.20} & \underline{84.14} & \underline{79.82} & \underline{80.32} & \underline{89.32} & 44.25 & 27.4 & 22.37 & 24.30 \\
    \hline
    8 & DeepSeek & 79.01 & 76.32 & 71.60 & 73.67 & 83.10 & 81.44 & 68.30 & 73.22 & 73.10 & 86.67 & 35.38 & \underline{29.10} & 28.72 & 26.57 \\       
    9 & AutoGen & 84.26 & 77.08 & 74.51 & 74.96 & 87.20 & 77.99 & 50.90 & 45.01 & 45.79 & 84.11 & 29.32 & 18.87 & 24.26 & 19.45 \\   
    10 & G-memory & \underline{86.52} & 77.32 & 78.41 & 75.46 & 88.45 & 82.45& 79.32 & 77.53 & 78.10 & 83.70 & 31.77 & 28.76 & 29.55 & \underline{28.10} \\
    \hline
    11 & OURS & \textbf{90.56} & \textbf{90.45} & \textbf{87.26} & \textbf{87.94} & \textbf{96.26} & \textbf{85.84} & \textbf{85.86} & \textbf{80.46} & \textbf{80.66} & \textbf{93.67} & \textbf{45.68} & \textbf{34.04} & \underline{30.71} & \textbf{29.32} \\
    \hline
    \end{tabular}%
}
\caption{Robustness evaluation on the \textbf{CJO2025} dataset.}
\label{tab:sota-comparison-cjo2025}
\end{table*}

\begin{table*}[t]
\centering
\label{tab:ablation}
\resizebox{\textwidth}{!}{%
    \begin{tabular}{l cc cc cc | cc cc cc}
    \hline
    \multirow{3}{*}{\textbf{Method}} & \multicolumn{6}{c|}{\textbf{CJO2025}} & \multicolumn{6}{c}{\textbf{CAIL2018}} \\
    & \multicolumn{2}{c}{\textbf{Law Article}} & \multicolumn{2}{c}{\textbf{Charge}} & \multicolumn{2}{c|}{\textbf{Prison Term}} & \multicolumn{2}{c}{\textbf{Law Article}} & \multicolumn{2}{c}{\textbf{Charge}} & \multicolumn{2}{c}{\textbf{Prison Term}} \\
    & \textbf{Acc} & \textbf{Ma-F} & \textbf{Acc} & \textbf{Ma-F} & \textbf{Acc} & \textbf{Ma-F} & \textbf{Acc} & \textbf{Ma-F} & \textbf{Acc} & \textbf{Ma-F} & \textbf{Acc} & \textbf{Ma-F} \\
    \hline
    vanilla & 82.12 & 76.54 & 77.61 & 72.10 & 27.06 & 19.76 & 73.04 & 72.01 & 67.95 & 69.13 & 26.07 & 25.01 \\  
    caseJudge & 83.08 & 78.83 & 79.21 & 71.68 & 28.17 & 22.18 & 76.40 & 75.52 & 70.80 & 72.18 & 24.14 & 25.25 \\ 
    \hline
    w/o Memory & 86.55 & 83.70 & 81.30 & 79.40 & 44.71 & 24.10 & 82.60 & 82.10 & 79.13 & 81.50 & 35.77 & \textbf{30.20} \\
    w/o MAS & 87.32 & 85.42 & 83.48 & \underline{80.32} & 39.50 & \textbf{30.15} & 83.10 & 81.50 & 79.80 & \underline{82.30} & 36.20 & 28.10 \\
    w/o DPO & 87.57 & \underline{87.37} & 82.60 & 79.17 & 42.77 & 28.40 & \underline{84.35} & 79.22 & \underline{81.70} & 79.20 & \underline{39.32} & 26.10 \\
    w/o $\mathcal{M}_{dir}$ & \underline{88.46} & 84.72 & \underline{84.32} & 80.16 & \underline{45.07} & 29.02 & 84.12 & \underline{83.01} & 80.30 & 79.77 & 38.32 & 27.87 \\
    \hline
    \textbf{SRM-LJP} & \textbf{90.56} & \textbf{87.94} & \textbf{85.84} & \textbf{80.66} & \textbf{45.68} & \underline{29.32} & \textbf{85.35} & \textbf{83.29} & \textbf{82.40} & \textbf{82.36} & \textbf{39.76} & \underline{29.08} \\
    \hline
    \end{tabular}%
}
\caption{Results of ablation experiments on CJO2025 and CAIL2018. The best results are \textbf{bolded} and the second-best are \underline{underlined}.}
\label{tab:abulation}
\end{table*}


\subsection{Baselines}
We compare SRM-LJP against representative baselines in four categories:

\vspace{0.5em}
\noindent \textbf{General Text Encoders.} 
Treating LJP as multi-label classification, \textbf{CNN} \cite{kim2014convolutional} uses convolution kernels for local feature extraction, while \textbf{BERT} \cite{devlin2019bert} leverages pre-trained Transformers for deep semantic understanding.

\vspace{0.5em}
\noindent \textbf{Dependency-Aware Models.} 
Modeling topological subtask dependencies, \textbf{MLAC} \cite{luo2017mlac} and \textbf{TopJudge} \cite{zhong2018topjudge} utilize attention mechanisms and DAGs, respectively. \textbf{MPBFN} \cite{yang2019mpbfn} employs a hierarchical forward-backward framework, while \textbf{EPM} \cite{Feng2022epm} enforces cross-task consistency via event-centric extraction.

\vspace{0.5em}
\noindent \textbf{Structure \& Knowledge-Enhanced Models.} 
\textbf{LADAN} \cite{xu2020ladan} and \textbf{CTM} \cite{liu2022ctm} apply graph distillation and contrastive learning to distinguish subtle legal nuances. \textbf{NeurJudge} \cite{yue2021neurjudge} and \textbf{R-Former} \cite{dong2021rformer} focus on fact decomposition and global consistency graphs, respectively. \textbf{PLJP} \cite{wu2023pljp} integrates domain models with retrieval-augmented generation (RAG).

\vspace{0.5em}
\noindent \textbf{LLMs and Agentic Systems.} 
All baselines in this category are equipped with RAG using the statutory library for fair comparison. \textbf{DeepSeek-V3.1} \cite{liu2024deepseek} serves as a zero-shot foundation model benchmark. \textbf{AutoGen} \cite{wu2024autogen} represents standard conversational multi-agent frameworks, while \textbf{G-memory} \cite{zhang2025gmemory} provides a graph-based memory mechanism for general-purpose agents.

==> sections/4.method.tex <==
\section{Method}
% 在本节中，我们提出 SRM-LJP（面向法律判决预测的自完善多智能体框架），这是一个旨在赋予 LJP 任务内在可解释性和动态自我完善能力的协作系统。具体而言，该框架由两个核心维度构成：
In this section, we present \textbf{SRM-LJP} (Self-Refining Multi-Agent Framework for Legal Judgment Prediction), a collaborative system designed to equip LJP tasks with both intrinsic interpretability and dynamic self-refining capabilities. Specifically, the framework is characterized by two core dimensions:\\
% 为了弥合通用 LLM 与严谨法理推演之间的差距，我们实施了一种渐进式司法逻辑对齐策略。首先，我们采用任务适配指令微调来确立基础判决能力并规范输出空间。随后，我们引入细粒度法理对齐（通过 DPO），利用自我反思衍生的对比数据，锐化模型在易混淆法律概念上的判别边界。由此生成的“司法专家”作为核心推理引擎，被嵌入到一个包含事件抽取、检索、起草、审查和决策的拓扑工作流中。这种显式的角色分工将隐式的判决过程转化为透明的、可交互的推理链条，从根本上增强了可解释性。
\vspace{0.5em}
\noindent\textbf{1. Expert-Led Interpretable Reasoning:} 
To bridge the gap between general LLMs and rigorous jurisprudential deduction, we implement a \textit{Progressive Judicial Logic Alignment Strategy}. We first employ \textit{Task-Adaptive Instruction Tuning} to establish foundational judgment capabilities and standardize the output space. Subsequently, we introduce \textit{Fine-Grained Jurisprudential Alignment} (via DPO), utilizing reflection-derived contrastive data to sharpen decision boundaries for confusing legal concepts. The resulting Judicial Expert serves as the core reasoning engine, embedded within a topological workflow comprising event extraction, retrieval, drafting, reviewing, and decision-making. This explicit role division transforms the implicit judgment process into a transparent, interactive reasoning chain, fundamentally enhancing explainability.\\
% 为了赋予多智能体系统持续学习和长尾泛化能力，我们构建了一个混合法理记忆系统 (HJM)。该架构的理论基础源于计算法学中的“微观指令范式” \citep{casey2016death}。传统法理学面临着刚性“规则”（清晰但僵化的法条）与模糊“标准”（灵活但充满噪声的先例）之间的两难困境。Casey 和 Niblett 提出，AI 可以通过处理海量数据打破这一二元对立，生成“微观指令”——即兼具标准的情境敏感性和规则的事前清晰性的精确规范。受此启发，我们的系统模拟了从“模糊标准”向“精确指令”的动态演进过程。通过将这些微观指令蒸馏为介于抽象法律与具体案例之间的中间模态，实现持续的知识精炼和对未见场景的适应性。
\vspace{0.5em}
\noindent\textbf{2. Self-Refining via Dual-Layer Memory:} 
To endow the multi-agent system with continual learning and long-tail generalization capabilities, we construct a \textbf{Hybrid Jurisprudential Memory (HJM)}. This architecture is theoretically grounded in the "Micro-Directive Paradigm" proposed by \citet{casey2016death} in computational law. Traditional jurisprudence faces a dilemma between rigid "Rules" (clear but inflexible statutes) and vague "Standards" (flexible but noisy precedents). ~\citet{casey2016death} posit that AI can bridge this dichotomy by processing massive data to generate "Micro-Directives"—precise norms that possess both the context-sensitivity of Standards and the ex-ante clarity of Rules. Inspired by this, our system simulates the dynamic evolution from fuzzy standards to precise directives. By distilling these Micro-Directives as an intermediate modality between abstract laws and specific cases, the system achieves continuous knowledge refinement and adaptivity to unseen scenarios.
\subsection{Domain-Specific Expert Alignment}
\subsubsection{Protocol-Aware Instruction Tuning}
While existing Large Language Models (LLMs) demonstrate robust capabilities in general text understanding, they exhibit deficiencies in grasping complex legal semantics. Consequently, relying solely on the inherent pre-trained knowledge of these models is insufficient for Legal Judgment Prediction tasks, which demand profound legal comprehension and reasoning abilities. To address this, we first employ a retrieval module to extract a candidate subset of legal articles $S=\{a_{i_1},a_{i_2},\ldots,a_{i_k}\}$ of size $k$ from the complete corpus of legal provisions $Y_a$, where $1\leq i_1,i_2,\ldots,i_k\leq m$. These candidate articles serve as auxiliary information and are fed into the expert LLM, denoted as $M_E$, alongside the factual description. The objective is to generate a predicted legal article $\hat{a}$ together with a relevant explanation $e_{\hat{a}}$ intended for human interpretation, formulated as $\hat{y}_a=(\hat{a},e_{\hat{a}})$. Furthermore, the generated explanations function as intermediate reasoning steps, enabling the LLM to perform self-reflection to refine its own predictions.

Formally, this process can be described as follows:
\begin{equation}
\hat{y}_a = M_E(s_d,a_{i_1},a_{i_2},\ldots,a_{i_k})
\end{equation}
To construct a high-quality instruction tuning dataset for legal article recommendation, we employ a data distillation strategy leveraging the relatively powerful Qwen2.5-14B. Specifically, we conduct inference on a sampled dataset $\mathcal{D}$ that encompasses all label categories. We then apply a strict filtering mechanism based on ground truth labels, exclusively retaining instances where the predicted legal article $\hat{a}$ aligns perfectly with the actual label. These verified samples constitute the training set for the Supervised Fine-Tuning (SFT) phase.
Concurrently, we compile the set of erroneous samples $D_{fault}$, which is reserved for utilization in subsequent training stages.
The training objective for SFT is defined as:
\begin{equation}
    \mathcal{L} = -\sum\limits_{(x,y)\in\mathcal{D}_{\mathrm{train}}} \log P(y \mid s_d, S)
\end{equation}
Given that the teacher model at this stage has not undergone specific training for legal article recommendation, the samples it correctly predicts represent relatively straightforward cases. Consequently, this fine-tuning phase aims to achieve the following two objectives:
Task Capability Alignment: Through supervised learning, the model preliminarily acquires the reasoning paradigm of leveraging the retrieved candidate set of legal articles () for recommendation tasks;
Output Space Standardization: We enforce the model to adhere to a specific structured output format. This standardization not only guarantees the parsability of the generated content but also lays the foundation for efficient inter-module communication within the subsequent multi-agent system.

\subsubsection{Logic-Driven Contrastive Alignment}

Given that Large Language Models (LLMs) lacking specialized training struggle to capture deep legal semantics, their initial predictions often exhibit significant deviations. To further align the model with legal adjudication logic, we leverage the previously collected error set $D_{fault}$ to design a Label-Guided Self-Reflection Mechanism, which automatically constructs the preference data required for DPO training. Specifically, we deploy the LLM as an autonomous agent. The agent initiates the process by generating an initial prediction $\hat y_{0}$ based on the case description and candidate legal articles. Subsequently, the system obtains binary feedback derived from the ground truth labels. For samples where the initial prediction $\hat y^{0}_{a}$ is incorrect, we prompt the LLM, denoted as $M_R$, to analyze logical loopholes and inaccurate legal reasoning within the prediction. Given the context of previous inputs and outputs, at each iteration $i$, $M_R$ leverages label information to provide detailed reflection advice $r^i_{\hat y_{i}}$, which functions as short-term memory. This advice $r^i_{\hat y_{i}}$ explicitly identifies deficiencies in the previous reasoning explanation $e^i_{\hat a}$, such as the omission of key constitutive elements, failure to distinguish between primary and secondary factors, disordered logical sequencing, or a focus solely on superficial content. Formally, this process can be described as follows:
\begin{equation}
r^i_{\hat y_{i}}= M_R(s_d,a_{i_1},a_{i_2},\ldots,a_{i_k},\hat y_i)
\end{equation}
Up to the current reflection iteration $i$, the accumulated reflection memory is denoted as $R^i_{\hat y_{i}} = [r^0_{\hat y_{0}},r^1_{\hat y_{1}},\ldots,r^i_{\hat y_{i}}]$. These reflections are combined with the original input information and fed into $M_E$, assisting in the generation of the correct legal article recommendation $\hat a_{i+1}$ alongside a more precise explanation $e^{i+1}_{\hat a}$. This process is formalized as:
\begin{equation}
\hat y^{i+1}_{a}= M_E(s_d,a_{i_1},a_{i_2},\ldots,a_{i_k},R^{i}_{\hat y_{i}})
\end{equation}
We extract "successfully corrected" samples from these interaction trajectories, defined as instances where an initially incorrect prediction was rectified following reflection. Based on these instances, we construct pairwise preference data by defining the preferred response as $\hat{y}_{w,a} = (\hat a_{\tilde{\boldsymbol{i}}-1},e_{\hat{a_{\tilde{\boldsymbol{i}}-1}}}) $ and the rejected response as $\hat{y}_{l,a} = (\hat a_{\tilde{\boldsymbol{i}}-1},e_{\hat{a_{\tilde{\boldsymbol{i}}-1}}}) $. Consequently, we compile the preference dataset $\mathcal{D}=\left\{\left(x^{(i)},y_w^{(i)},y_l^{(i)}\right)\right\}_{i=1}^N$. Finally, utilizing the SFT-trained model as the reference, we employ the DPO algorithm to perform parameter updates:

\begin{equation}
\resizebox{0.95\hsize}{!}{$
\mathcal{L}(\pi_\theta; \pi_{\text{ref}}) = -\mathbb{E}_{\mathcal{D}} \left[ \log \sigma \left( \beta \log \frac{\pi_\theta(y_W|x)}{\pi_{\text{ref}}(y_W|x)} - \beta \log \frac{\pi_\theta(y_l|x)}{\pi_{\text{ref}}(y_l|x)} \right) \right]
$}
\end{equation}
\subsection{Topological Multi-Agent Judicial Workflow}
\label{sec:workflow}

In real-world scenarios, Legal Judgment Prediction (LJP) is never an isolated classification problem but a complex collaborative process covering case filing, research, drafting, deliberation, and final adjudication. To replicate this rigorous procedure, we design a multi-agent system to simulate a real-world \textbf{Virtual Collegial Panel}. This architecture assigns distinct jurisprudential roles to heterogeneous agents, ensuring the decision-making process adheres to the procedural justice of the Chinese criminal court system.

\subsubsection{System Topology and Role Definition}

We formally define the judicial judgment prediction system as a collaboration system based on a Directed Acyclic Graph (DAG), denoted as $\mathcal{M}=\langle\mathcal{U},\mathcal{A},\mathcal{S},\mathcal{P},\Phi\rangle$, where:
\begin{itemize}[leftmargin=*, nosep]
    \item $\mathcal{U}$: The input space, representing the raw textual description of the case facts.
    \item $\mathcal{A}=\{a_{clerk}, a_{assist}, a_{case}, a_{super}, a_{pres}\}$: The set of specialized agents constituting the panel.
    \item $\mathcal{S}$: The state space, comprising the intermediate structured outputs generated by agents in the reasoning chain.
    \item $\mathcal{P}$: The pre-defined graph-based workflow that dictates the node scheduling mechanism.
    \item $\Phi$: The unified communication protocol.
\end{itemize}

Each agent $a_{i} \in \mathcal{A}$ is modeled as a conditional probability distribution $\pi_i(o_i|I_i)$, where $I_i$ represents the contextual input for the node and $o_i$ denotes the output. Specifically, the discriminative agent (Case-handling Judge) is parameterized by the domain-expert model $\pi^*_{\theta}$, which was aligned via semantic legal tuning in the previous stage. We define a context assembly function $\Psi(\cdot)$ to construct the prompt for each agent.

The inference process evolves through the following specialized roles:

\vspace{0.5em}
\noindent \textbf{1. Court Clerk ($a_{clerk}$)}
Acting as the foundation of the workflow, the Court Clerk is responsible for pre-processing the raw case dossier. To mitigate noise and disentangle complex narratives, the clerk extracts key factual points (e.g., subjective criminal intent, specific criminal acts, and consequences) from the unstructured text $u \in \mathcal{U}$. This process is formulated as:
\begin{equation}
o_{ext} \sim \pi_{clerk}(\cdot \mid u)
\end{equation}
where $o_{ext}$ represents the denoised, structured factual description.

\vspace{0.5em}
\noindent \textbf{2. Judicial Assistant ($a_{assist}$)}
The Judicial Assistant acts as the bridge to the legal knowledge base. Its goal is to provide reliable standard statutory grounds for the trial by querying the statutory library $\mathcal{D}_{law}$. 
First, based on $o_{ext}$, it retrieves the Top-$K$ relevant articles via dense vector retrieval:
\begin{equation}
S_{vector} \leftarrow \text{Search}(q=o_{ext}, \mathcal{D}=\mathcal{D}_{law}, k=K)
\end{equation}
Then, leveraging the agent's strong semantic understanding capabilities, it filters $S_{vector}$ to select $N$ highly relevant articles, constituting the reliable candidate set of reference statutes $S_{statute}$, where $|S_{statute}| = N \le K$:
\begin{equation}
S_{statute} \sim \pi_{assist}(\cdot \mid \Psi(o_{ext}, S_{vector}))
\end{equation}

\vspace{0.5em}
\noindent \textbf{3. Case-handling Judge ($a_{case}$)}
This component is the core reasoning engine, forming an iterative loop with the Adjudication Supervisor. The Case-handling Judge first generates a preliminary judgment by synthesizing the case facts $o_{ext}$ and the retrieved statutes $S_{statute}$. 
Let $t$ denote the iteration round, and $h_t$ represent the feedback provided by the supervisor for the previous round (where $h_0$ is null):
\begin{equation}
y_{draft}^{(t)} \sim \pi^*_{\theta}(\cdot \mid \Psi(u, o_{ext}, S_{statute}, h_{t}))
\end{equation}
Here, $\pi^*_{\theta}$ utilizes the fine-grained legal semantic discriminative ability acquired during training to pinpoint the optimal legal article from $S_{statute}$ and provide a jurisprudential explanation. \textbf{Note that this process strictly relies on statutes and does not involve accessing precedents or micro-directives from the memory system.}

\vspace{0.5em}
\noindent \textbf{4. Adjudication Supervisor ($a_{super}$)}
To ensure the judgment is not only legally valid but also appropriate, the Adjudication Supervisor intervenes. Unlike the Drafter, this agent has privileged access to the full \textbf{Hybrid Jurisprudential Memory}. It utilizes judicial precedents $S_{std}$ from the \textit{Contextual Standards Archive} ($\mathcal{M}_{std}$) and relevant micro-directives $S_{dir}$ from the \textit{Evolving Micro-Directive Base} ($\mathcal{M}_{dir}$).
Armed with this tacit knowledge, $a_{super}$ strictly scrutinizes the draft $y_{draft}^{(t)}$. If discrepancies are found (e.g., compliant with statutes but violating a micro-directive on sentencing), it issues a rejection signal with corrective advice:
\begin{equation}
\begin{split}
(flag_t, fdbk_t) \sim \pi_{super}(\cdot \mid \Psi(u, y_{draft}^{(t)}, \\
 \quad S_{statute}, S_{std}, S_{dir}))
\end{split}
\end{equation}
where $flag_{t} \in \{\mathsf{Pass}, \mathsf{Reject}\}$ is the decision signal, and $fdbk_{t}$ is the suggestion in natural language (e.g., Incorrect charge qualification, omission of key elements).
The system updates the state based on $flag_{t}$:
\begin{equation}
h_t \leftarrow h_{t-1} \oplus fdbk_t
\end{equation}
The operation flow is defined as:
\begin{equation}
\text{Op} =
\begin{cases}
    \text{to verdict}, & \text{if } flag_t = \text{Pass} \lor t \ge T_{max} \\
    \text{redraft}, & \text{if } flag_t = \text{Reject}
\end{cases}
\end{equation}

\vspace{0.5em}
\noindent \textbf{5. Presiding Judge ($a_{pres}$)}
Finally, the Presiding Judge aggregates the refined draft and the comprehensive context to render the final verdict. As the ultimate decision-maker, $a_{pres}$ also possesses the capability to access the full memory bank to ensure global consistency:
\begin{equation}
y_{final} \sim \pi_{pres}(\cdot \mid \Psi(u, S_{statute}, S_{std}, S_{dir}, y_{draft}^{(final)}))
\end{equation}

% 基于前述的‘微观指令范式’，本节详细阐述混合法理记忆（HJM）的物理架构。我们将抽象的法理概念实体化（Instantiate）*为具体的计算组件：将刚性的‘规则’映射为不可变的*法条库，将模糊的‘标准’映射为情境标准归档，并将动态的‘微观指令’实例化为演化微指令库。这种架构设计使得系统能够自动完成从标准到指令的知识蒸馏。我们将该记忆系统形式化为一个四元组 
\subsection{The Hybrid Jurisprudential Memory (HJM)}
Building upon the aforementioned "Micro-Directive Paradigm", this section details the architectural implementation of the Hybrid Jurisprudential Memory (HJM). We \textbf{operationalize} the abstract jurisprudential concepts into concrete computational components: mapping rigid "Rules" to the immutable \textbf{Statutory Library}, vague "Standards" to the \textbf{Contextual Standards Archive}, and dynamic "Micro-Directives" to the \textbf{Evolving Micro-Directive Base}. This design enables the system to automatically execute the knowledge distillation process from Standards to Directives.

Formally, we define the memory system as a 4-tuple $\mathcal{M} = \langle \mathcal{M}_{std}, \mathcal{M}_{dir}, \mathcal{D}_{law}, \Phi_{trans} \rangle$, where:
\begin{itemize}[leftmargin=*, nosep]
    \item $\mathcal{M}_{std}$ (\textbf{Contextual Standards Archive}): Stores granular historical adjudication trajectories, representing legal "Standards"
    \item $\mathcal{M}_{dir}$ (\textbf{Evolving Micro-Directive Base}): Stores distilled judicial experiences, representing "Micro-Directives."
    \item $\mathcal{D}_{law}$ (\textbf{Statutory Library}): Stores immutable criminal statutes, serving as hard constraints.
    \item $\Phi_{trans}$ (\textbf{Translation Strategy}): The mechanism for micro-directive generation and updating.
\end{itemize}

\subsubsection{The Contextual Standards Archive ($\mathcal{M}_{std}$)}
We design this layer as an undirected attributed graph $\mathcal{G}_{std}=(\mathcal{V},\mathcal{E},\mathcal{F}_{sim})$. Each node $v_i \in \mathcal{V}$ is not merely a document but encapsulates the \textbf{complete adjudication trajectory} of a case within the virtual collegial panel, serving as an empirical Legal Standard:
\begin{equation}
v_i=\langle\mathrm{txt}_i, \mathbf{h}_i, \Lambda_i, c_i\rangle
\end{equation}
where $\mathrm{txt}_i$ records the full factual and reasoning chain, preserving the granularity of judicial practice; $\mathbf{h}_i$ denotes the normalized dense vector embedding; $\Lambda_{i}=\{\mathcal{L}_{art},\mathcal{L}_{acc}\}$ represents legal metadata (statutes and charges); and $c_i$ is the cluster identifier assigned by the FINCH algorithm.

\textbf{Contextual Association:} An edge $e_{i,j}$ exists between two nodes if and only if they share sufficient semantic and legal similarity:
\begin{equation}
(v_i,v_j)\in\mathcal{E} \Longleftrightarrow \mathrm{sim}(\mathbf{h}_i,\mathbf{h}_j) \geq \tau \wedge (\Lambda_i \equiv \Lambda_j)
\end{equation}
The similarity metric $\mathcal{F}_{sim}$ is defined as $\mathcal{F}_{sim}(\mathbf{h}_i,\mathbf{h}_j) = \mathbf{h}_i^\top\mathbf{h}_j \approx 1-\mathrm{dist}_{cosine}(\mathbf{h}_i,\mathbf{h}_j)$.

\subsubsection{The Evolving Micro-Directive Base ($\mathcal{M}_{dir}$)}
This layer maintains a set of dynamically evolving \textbf{Judicial Experiences}, organized by clusters. Each micro-directive unit $m_{dir}$ is defined as:
\begin{equation}
m_{dir} = \langle r_{txt}, \mathcal{S}_{conf}, \mathcal{C}_{pos}, \mathcal{C}_{neg}, \Lambda_{anchor} \rangle
\end{equation}
\begin{itemize}[leftmargin=*]
    \item $r_{txt}$: The micro-directive in natural language. It is not a broad statute but a precise interpretation of law in a specific context. 
    \item $\mathcal{S}_{conf}$: The confidence score of the directive.
    \item $\mathcal{C}_{pos/neg}$: Traceable indices pointing to supporting or conflicting cases in $\mathcal{M}_{std}$.
    \item $\Lambda_{anchor}$: The \textbf{Statute Anchor} (e.g., Article 114), ensuring the directive adheres to the standardized law.    \begin{quote}
    \textit{Example:} For Article 114 (Endangering Public Safety), a stored directive might specify: Subjective motives (e.g., wage demands) do not negate the objective crime; acts like wrong-way driving on highways constitute this crime equivalent to arson.
    \end{quote}
\end{itemize}

\subsubsection{Evolutionary Mechanism and Lifecycle Management}
To realize the evolution from coarse-grained imitation to fine-grained understanding, we design a lifecycle strategy encompassing archiving, retrieval, and hybrid distillation.
\begin{figure}[t]
    \centering
    % 这里的 scale 或者 width 根据实际情况微调
    \includegraphics[width=0.95\linewidth]{figs/evo.pdf} 
    
    \caption{\textbf{The evolutionary lifecycle of Micro-Directives.} 
    The process consists of three phases: 
    (A) \textit{Inductive Generation} clusters raw cases to form initial rules; 
    (B) \textit{Contrastive Refinement} sharpens legal boundaries by contrasting success ($T^+$) and failure ($T^-$) samples; 
    (C) The finalized directive is stored in the \textit{Micro-Directive Base} with a confidence score.}
    
    \label{fig:evolution_process}
\end{figure}

\vspace{0.5em}
\noindent \textbf{1. Standard Archiving (Memory Generation).}
Upon inference conclusion, the system validates the result $y_{final}$ against the ground truth $\ell_{gt}$. If all three subtasks are correct, the full trajectory is written into $\mathcal{M}_{std}$ as a new Standard Precedent:
\begin{equation}
\Phi_{archive}(u) = 
\begin{cases}
    \mathrm{Embed}(u, y_{\text{final}}), & \text{if } y_{\text{final}}= \ell_{\text{gt}} \\
    \bot, & \text{otherwise}
\end{cases}
\end{equation}
This append-only process preserves the empirical reality, ensuring the purity of the experience pool.

\vspace{0.5em}
\noindent \textbf{2. Contextual Retrieval and Injection.}
To prevent cross-domain contamination, we design a multi-dimensional relevance scoring mechanism. Let $S_{statute}$ be the candidate statutes retrieved for the current task. The score for a memory unit $m$ is:
\begin{equation}
\begin{split}
    \mathrm{Score}(m) = & \, \alpha \cdot \mathrm{IoU}(\Lambda_m, S_{statute}) \\
    & + \beta \cdot \mathrm{Topo}(m, \mathcal{N}_{graph}) \\
    & + \gamma \cdot \mathrm{SemSim}(m, u_{curr})
\end{split}
\end{equation}
\begin{itemize}[leftmargin=*]
    \item \textbf{IoU (Statute Anchor):} $\frac{|\Lambda_{m}\cap S_{statute}|}{|\Lambda_{m}\cup S_{statute}|}$. Unlike general text retrieval, this enforces consistency in legal applicability, supporting cross-scenario analogical reasoning.
    \item \textbf{Topo (Topological Co-occurrence):} Indicates whether $m$ appears in the activation diffusion path from the current case. If a precedent is jointly referenced by neighbors, it signifies core knowledge, enabling associative retrieval.
    \item \textbf{SemSim (Semantic Similarity):} Captures factual proximity between $m$ and the current case $u_{curr}$.
\end{itemize}

\vspace{0.5em}
\noindent \textbf{3. Micro-Directive Generation and Evolution.}
When new nodes in $\mathcal{M}_{std}$ reach a threshold $B$, the translation process is triggered via a three-stage mechanism:

\textbf{Phase A: Inductive Generation.}
The system operates on homogeneous clusters $\mathbf{C}$ obtained via manifold partitioning. For a batch of \textbf{successful precedents} $V_{batch}$ within a cluster, the Meta-LLM identifies common adjudication patterns to execute the \textbf{ADD} operation:
\begin{align}
    \Delta_{ind} = & \, \mathrm{LLM}_{meta}\left( \bigcup_{v \in V_{batch}} \mathrm{txt}(v) \mid \mathrm{Prompt}_{induce} \right) \notag \\
     & \Rightarrow \textbf{ADD}(r_{new})
\end{align}
This mimics the emergence of new directives from consistent rulings.

\textbf{Phase B: Contrastive Refinement.}
To clarify boundaries, the system constructs \textbf{Success vs. Failure} pairs ($T^+$ vs. $T^-$) under strict label co-domain constraints. The LLM analyzes differences to execute \textbf{REFINE/PRUNE}:
\begin{align}
    \Delta_{con} = & \, \mathrm{LLM}_{meta}\big( T^+, T^-, \mathcal{M}_{dir} \mid \mathrm{Prompt}_{diff} \big) \notag \\
    & \Rightarrow \{\textbf{REFINE}, \textbf{PRUNE}\}
\end{align}
This mimics trial-and-error to correct applicability conditions (e.g., clarifying that subjective motives do not affect objective conviction).

\textbf{Phase C: Doctrinal Consolidation.}
To prevent fragmentation, the system periodically triggers consolidation. It clusters $\mathcal{M}_{dir}$ and splits them by exact label matching. The LLM then rewrites multiple directives in a sub-group into a robust rule and accumulates confidence:
\begin{equation}
\begin{split}
    m_{merged} &= \mathrm{Compress}(G_{sub}); \\
    \mathcal{S}_{conf}(m_{merged}) &\leftarrow \sum_{m \in G_{sub}} \mathcal{S}_{conf}(m)
\end{split}
\end{equation}
This cycle ensures the entropy reduction from fragmented directives to systematic judicial experience.
